PIE-NET: Parametric Inference of Point Cloud Edges

We introduce an end-to-end learnable technique to robustly identify feature edges in 3D point cloud data. We represent these edges as a collection of parametric curves (i.e.,lines, circles, and B-splines). Accordingly, our deep neural network, coined PIE-NET, is trained for parametric inference of edges. The network relies on a "region proposal" architecture, where a first module proposes an over-complete collection of edge and corner points, and a second module ranks each proposal to decide whether it should be considered. We train and evaluate our method on the ABC dataset, a large dataset of CAD models, and compare our results to those produced by traditional (non-learning) processing pipelines, as well as a recent deep learning based edge detector (EC-NET). Our results significantly improve over the state-of-the-art from both a quantitative and qualitative standpoint.

==> 3_method_OLD.tex <==
\subsection{Overview}
\label{sec:overview}
Please refer to Figure~\ref{fig:pipeline} for an overview of our algorithm pipeline. 
Given a 3D point cloud, we firstly divide the point sets into blocks through voxel partition (Section~\ref{sec:PatchNet}). Each block is then segmented by Patch-Net (Section~\ref{sec:PatchNet}). Then, for each model, we search out the adjacent segments in the adjacent blocks, and form the candidate merge pairs (Section~\ref{sec:MergeNet}). Subsequently, each candidate merge pair is fed into a Merger-Net which predicts the match score that they belong to the same part (Section~\ref{sec:MergeNet}). 
Finally, a merge graph is constructed, and each node in the graph refers to the predicted segment from Patch-Net, and the edge refers to the matching score from Merge-Net between the two segments.
According to the merge graph, we design a bottom-up hierarchical aggregation algorithm to obtain the final fine-grained parsing result (Section~\ref{sec:labelling}).
In the next, we describe the three algorithmic components, including Patch-Net, Merge-Net, and hierarchical aggregation algorithm for fine-grained parsing.



, and is composed of three modules: a \textit{edge} and corner \textit{points} detection module (\Section{detection}), a \textit{open} curve module (\Section{open_gen}), and a \textit{closed} curve module (\Section{closed_gen}).
A generated curve can fall into two categories: open or closed curve.
An closed curve is a curve where the beginning and end points \AT{corners} are different, and a closed curve where they are the same.

In the detection module, we adopt the focal loss to detect edge and corner points, which are usually very sparse in the point cloud.
For open curve estimation, we can consider each pair of corner points as a open curve start and end point.
Then each pair of corner points pass through the open curve proposal module to sample the relevant edge points and to generate a  parametric curve.
For \textit{closed} curve, we first sample edge points uniformly to get a subset that can be considered closed seed points.
For each seed point, through closed curve proposal module, we can generate a closed curve and score the confidence of the curve.  Finally, we design a simple curve selection algorithm to merge all the curves to generate the final fitting result.

Because the point cloud contains much noise, for each edge point, we regress the minimum distance vector from it to groud truth curve. Similarly, for each detected corner point, we also regressed the residual vector from it to the groud truth corner points.


+ \lambda_{corner_cls}L_{corner_cls} + \lambda_{corner}_{cls}L_{corner}_{reg}
\paragraph{\textbf{edge points detection loss $L_{edge}$}}
where the first term is for edge points classification, and the second term is for the edge-to-curve distance vector regression.
$\hat{T_e}$ is the predicted probability of each point being a edge point and $T_e$ is the ground truth.

This can lead to a serious class imbalance, which will seriously hinder the classification result.
Instead of cross entropy loss function, we adopt the focal loss function [He ICCV 2017], which is a dynamically scaled cross entropy loss for dealing with edge point classification.

\paragraph{\textbf{corner points detection loss $L_{edge}$}}
Similarly, corner points detection loss $L_{corner}$ is defined as:
where we also use focal loss and smooth $L_1$ loss for corner classification $L_\text{cls}$ and residucal vector regression $L_\text{reg}$. We set $\lambda_{c}$ = 100.

according to the corner points classification and the corresponding residual vector. After that, The corner point detected by the network are clustered into groups, within which the distance between arbitrary two corner points is no greater than $dis$, 
and all the points with the highest probability in their groups are predicted as corner points.
We use $\delta=0.01$ all ourexperiments.

\subsubsection{Corner Pair Sampling}
\label{sec:open_edge_segmentation}
% 
\todo{For each corner pair, to generate an open curve, we first need to find as many edge points related to this open curve as possible.
It is easy to know that there is a high probability that the relevant curve points will appear in the space formed by the two corner points.
In this paper, ball sampling is adapt by taking the midpoint of two corner points as the center and half of the distance as the radius, and samples a fixed-cardinality subset from the set of edge points.
For the set of points sampled from each corner pair, we call it $corner$ $pair$ $ball$.
Though simple, this sampling technique is easy to integrate into an end-to-end pipeline and works well in practice.} \AT{I do not understand -- at all}.

We first combine the corner points to generate a set of corner points pairs $\{p_i = \{{c_i}_1,{c_i}_2\}|{c_i}_1,{c_i}_2 \in C\}$. A shared sampling module samples edge points from each corner pair independently. Specifically, for each corner pair $p_i$, we sample a subset of $K$ edge points using farthest point sampling based on the midpoint $center_i$ and half the distance $distance_i$ of corner points in 3D Euclidean space, to get
$\{{p_i}_k\}_{i=1}^K$ where ${p_i}_k \in E$.

% \subsubsection{Curve Generation}
% \label{sec:open_edge_segmentation}
% In the second part of the Open Curve Proposal Generation (OCPG), the $corner$ $pair$ $ball$ from corner pair sampling
% module are further processed to segment the relevant curve points from the initial sampling points $\{{p_i}_k\}_{i=1}^K$, identify the curve type, and estimate the curve parameters.
% From each $corner$ $pair$ $ball$, OCPG first extract points features, which then are fed through a shared PointNet-based segmentation, classification, and regression sub-network.
% The segmentation is obtained by predicting a per-point binary mask to indicate whether it belongs to the current curve,
% and curve parameters are refined by measuring the relative deviation between the predicted parameterized curve and ground truth curve. 

% We visualie the architecture of Open Curve Proposal Generation (OCPG) in Figure XXX.
% Given a $corner$ $pair$ $ball$ $p = \{p_1,...,p_K\}$, OCPG is trained to minimize a multi-task loss function defined within each $corner$ $pair$ $ball$ as:
% \begin{equation} 
%   L = L_\text{mask}(M_p,\hat{M_p}) + L_\text{cls}(T_p, \hat{T_p}) + L_\text{para}
% \label{eq:open_curve_gen_loss}
% \end{equation}
% where the first term is for sampling points segmentation, the second term is for curve type classification, and the final term is for curve parameters estimation. 
% $M_p$ and $\hat{M_p}$ are ground truth and predicted binary mask, respectively.
% $T_p$ and $\hat{T_p}$ are ground truth and predicted curve type label, respectively.
% $L_\text{mask}(\centerdot)$ and $L_\text{cls}(\centerdot)$ are all softmax cross-entropy loss.
% $L_\text{para}(\centerdot)$ is chamfer distance loss, which is used to measure the relative deviation between the generated parameterized curve and the ground truth.

% Curve parameters loss $L_{para}$ is defined as:
% \begin{equation}
%  L_\text{para} = {T_p}_c*L_\text{c}+ {T_p}_b*L_\text{b} + {T_p}_l*L_\text{l}
% \label{eq:l_edge}
% \end{equation}
% where  $L_\text{c}$, $L_\text{b}$ and $L_\text{l}$ represent different curve type (Cycle, B-Spline and Line) parameters estimation, respectively. ${T_p}_c$, ${T_p}_b$ and ${T_p}_l$ are the ground truth labels of three different curves.
% Next, we explain design details about these three curve parameters loss.

\paragraph{\textbf{Circle Loss $L_\text{c}$}}

The cycle loss is defined as:
\begin{equation}
 L_\text{c} = L_\text{CD}(C_p, \hat{C_p})
\label{eq:l_edge}
\end{equation}
where $C_p$, $\hat{C_p}$ are the sampling point sets from predicted cycle parameters $\hat{C}$ and ground truth $C$.
$L_\text{CD}(\centerdot)$ is chamfer distance between two point sets.


Similarly, the endpoints of the fitted line pass through two corner points, so network only predict their residual vectors $\Delta{P_1}$ and $\Delta{P_2}$.
The Line loss is defined as:
\begin{equation}
 L_\text{l} = L_\text{CD}(L_p,\hat{L_p})
\label{eq:l_edge}
\end{equation}
where $L_p$, $\hat{L_p}$ are the sampling point sets from predicted line parameters $\hat{L}$ and ground truth $L$.
$L_\text{CD}(\centerdot)$ is chamfer distance between two point sets.

\paragraph{\textbf{B-Spline Loss $L_\text{b}$}}
We represent a B-Spline curve by $\beta = (P, N)$ where $P_i{(i=0,1,...,n)}$ are control points. $N_{i,k}{(t)}$ (i=0,1,...,n) are the $i$-th B-Spline basis function of order $k$.
A B-Spline curve is parametrized by:
\begin{equation}
 P_{{t}} = \sum_{i=0}^n{P_iN_{i,k}(t)}
\label{eq:l_edge}
\end{equation}
 
where, in our work, we use cubic B-spline curve, and we set $n = 4$.
At the same time, in order to retain the endpoint property of the fitted curve, we use quasi-uniform B-Spline.
It has the start-knot and end-knot have repetitiveness of $k$, which means the start point and end point of curve are the same as the start point and end point of the control points.


The B-Spline loss is defined as:
\begin{equation}
 L_\text{b} = L_\text{CD}(B_p, \hat{B_p})
\label{eq:l_edge}
\end{equation}
where $B_p$, $\hat{B_p}$ are the sampling point sets from predicted  parameters $\hat{B}$ and ground truth $B$.
$L_\text{CD}(\centerdot)$ is chamfer distance between two point sets.

Note that, since we need the fitting B-Spline curve through the corner points.
For the first and last endpoints, we only estimate the residual vector $\Delta{{P_c}_1}$ and $\Delta{{P_c}_k}$.
Then, we can obtain all predicted control points $\hat{B} = \{\hat{P_i}\}$ where $\hat{P_1} = {P_c}_1 + \Delta{{P_c}_1}$ and
$\hat{P_k} = {P_c}_k + \Delta{{P_c}_k}$.


% --- Circle
\paragraph{Circular arc parameterization}
We parameterize circular \textit{arcs} as $\beta {=} (n, c, r)$, where $n$ is the normal of the circle, and $c$ and $r$ are its center and radius.
We then randomly sample points on the circle, and express them as a function of~$\beta$.
To achieve this, we draw $\alpha \in [0, 2*\pi]$, and generate random samples $p(\alpha | \beta)=c + r(u cos(\alpha) + v sin(\alpha)$, \todo{where $u=...$ and $v=...$.}
\AT{u,v need to be a expressed as a function of $n$ for this to be differentiable? How do you do that?}
\AT{ohhhh... you only do arcs of circle here.. then the $[0,2\pi]$ would not work... so what do you do?}

For closed curve proposal generation, we adopt a similar idea: grouping + fitting.
\Figure{closednet} illustrates our closed curve proposal generation network. 
The entire network can be split into two parts:
one that processes edge points to generate closed points proposal; 
and the other part that operates on these proposals to estimate curve parameters and regress confidence score for each proposal.
Note that, in this work, we handle only one type of closed curve, i.e., circle.

\paragraph{\textbf{Closed Points Grouping}}
Unlike an open curve, which is determined by two corner points, the number of closed curves in the point set is unknown.
For closed points grouping, we therefore opt for a proposal-based solution.
Inspired by SGPN (Similarity Group Proposal Network) [xxxxx], we can consider that the points features within the same closed curve have stronger similarity, 
at the same time, the features of points between different curves should be as dissimilar as possible. 
According to this idea, we defined a similarity matrix $S \in N \times N$ to describe this phenomenon.
$N$ represents the number of point sets. 
Each entry $S_{ij}$ in the similarity matrix $S$ indicates whether two points, $p_i$ and $p_j$,  belong to the same closed curve.   
Each row can then be viewed as a proposal. 

The similarity loss $L_\text{sim}$ is defined as:
\begin{equation}
  L_\text{sim}=\sum_{p_i,p_j\in P, i\neq j}S_{i,j},
\label{eq:simloss}
\end{equation}
where
$$ S_{i,j}=\left\{
\begin{array}{rcl}
\||F(p_i)-F(p_j)\||_2,     &      {l(i,j)=1}\\
\max\{0,K-\||F(p_i)-F(p_j)\||_2\},      & {l(i,j)=0}
\end{array} \right. $$
where $l(i, j)$ indicates whether $p_i$ and $p_j$ belong to the same closed curve in the ground-truth 
(1 means $yes$). 
$F$ is point-wise feature computed with PointNet++. 
$K$ is a constant that controls the degree of dissimilarity points in different parts; we use $K = 100$ by default. 

\paragraph{\textbf{Closed Curve Fitting}}
Closed Curve Fitting(CCF) takes each proposal as input and regresses a closed curve $\beta$.
CCF first samples 3 points $\{p_1,p_2,p_3\}$ from each proposal with Farthest Points Sampling (FPS), where $p_1$ is the corresponding seed point.
The module then employs a PointeNet which processes each proposal and outputs a feature vector $f_p$, 
feed the feature through a multi-layer perceptron (MLP), and regresses 3 residual vector 
$\{\Delta_1,\Delta_2,\Delta_3\}$ for 3 sampling points. 
We can get the closed curve $\beta = \{p_1 + \Delta_1,p_2 + \Delta_2,p_3 + \Delta_3\}$.  
CCF takes an additional MLP taking $f_p$ predicting closed proposal confidence score (good closed proposal/not) for each proposal. 
The confidence score is supervised with ground truth segmentation;
positive proposals come from seed points belonging to closed curve, 
and their overlap with some ground truth closed points segmentation with an intersection over union (IoU) larger than 0.5.   
Negative proposals are those whose IoUs with all the ground truth boxes are less than 0.5.


\paragraph{\textbf{Losses}}
The network is trained to minimize a multi-task loss function.
$L_{closed}$ defined for each potential closed curve proposal.
$L_{closed}$ is a summation of three terms including the closed points grouping loss $L_{sim}$, 
closed curve parameters estimation loss $L_{closed}$ and confidence socre loss $L_{score}$.
More formally:
% 
\begin{equation} 
   \loss{closed} = \loss{sim}(S_p,\hat{S}_p) + \loss{score}(C_p, \hat{C}_p) + \loss{para}(\beta)
\label{eq:open_curve_gen_loss}
\end{equation}
where $S_p$ and $\hat{S}_p$ are the ground truth / predicted similarity matrix, $C_p$ and $\hat{C}_p$ are ground truth / predicted confidence score for each proposal, and $\beta$ the closed curve parameters.
We use $L_2$ loss for both $\loss{sim}(\centerdot)$ and $\loss{score}(\centerdot)$. While for regression:
% 
\begin{equation}
\loss{para} 
=
T_\text{circle} \cdot \loss{circle}(\beta)
\end{equation}
% 
Where $T_*$ is the ground truth one-hot labels for the seed points, while $L_*$ are Chamfer Distance losses measuring the expectation of euclidean deviation between the closed curve having parameters $\beta$ and the ground truth.
In order to compute expectations, we need to draw random samples from closed curve which are \textit{parametric} in the degrees of freedom $\beta$.


\subsection{Curve proposal selection}
\label{sec:selection}

\paragraph{\textbf{Open Curve Selection}}
For the open curve, because the corner points detected by network are redundant, many redundant short curves are predicted, as shown in figure XX. 
Therefore, we design a simple selection strategy based on segmentation of corner pairs.
We prune segmentations into clean, non-overlapping open curves by applying a simple metric $O(A,B) {=} max\{I(A,B)/A, I(A,B)/B\}$, where $A$ and $B$ are two corner pair segmentatons, I(.) represents the intersection of two point sets;
segmentations with $O$ greater that $Th_o$ are merged together by selecting the segmentation with the larger area, 
and the corresponding open curve is selected.

\paragraph{\textbf{Closed Curve Selection}}
For closed curve selection, we also use a simple selection strategy based on segmentation.
The similarity matrix S produces N closed group proposals, 
many of which are non-closed curve or represent the same closed curve. 
We first discard proposals with predicted confidence score less than $Th_p$.  
We further prune our proposals into clean, non-overlapping closed proposals by applying Non-Maximum Suppression; 
groups with IoU greater than $Th_M$ are merged together by selecting the group with the maximum confidence score.
Finally, for each closed segmentation, we select a closed curve with the maximum matching.
We use Chamfer Distance measuring the expectation of euclidean deviation between the closed curve and the closed segmentation.







==> 4_results_OLD.tex <==
\section{Results and evaluation}
\label{sec:results}
% 
We evaluate the performance of our work by performing ablation studies, as well as comparing against both traditional and learnt pipelines for edge detection.

\paragraph{Metrics}
To evaluate edge classification we measure precision/recall and the IoU between predictions, while to evaluate the geometric accuracy of the reconstructed edges we employ the Edge Chamfer Distance introduced by~\citeN{bspnet}.
Note that, differently from~\citeN{bspnet}, we \textit{do not} need to process the dataset to identify ground truth edges, as these are provided by the dataset.

\input{fig/ablation.tex}
\subsection{Ablation studies -- \Figure{ablation}}
In this section, 
We use the following four metrics to measure network performance.
Where, $ECD$ represents the chamfer distance between the curve predicted by the network 
and the GT curve; $IOU$, $Pricision$ and $Recall$ represent the segmentation performance.

\paragraph{Sphere radius}
When performing Open curve proposal generation (Section 3.4), 
sphere radius , sampled edge points for each corner pair is an important parameter of our method.
According to observation, we found that a large probability of curve points were scattered in the space enclosed by two corner points.
In our work, we set the radius to be half of the distance between the two corner points.
To verify this, we designed a scale to enlarge the radius of the sphere.
We experiment the parameter settings $scale$ being set to 1.5and 3 respectively, while keeping all other parameters unchanged.

The results are shown in Figure XXX. 
As the radius of the sphere increases, it is difficult to clearly analyze the corresponding curve points 
because of the large amount of noises introduced. 
So the predicted curve quality is very poor.
It shows that our hypothesis is completely valid.

\paragraph{$\tau_c$}
In Figure xx, we also study curve generation performance over the change of the parameter $\tau_c$.
We experiment with the parameter  $\tau_c$ of 0.8 and 0.95, while keeping all other parameters the same.
In this work, this parameter is set to 0.9.
We report the performance in our testing set, see Figure XXX.
We find that the curve generation quality grows slight as the parameter $\tau_c$ increases.
This shows that our network is insensitive to the corner points.
When the threshold is too large, the quality of curve generation begins to decline.
This is because some high-quality corner points are filtered out when the parameters are too large, resulting in the absence of some curves.

\subsection{State-of-the-art comparisons \Figure{star}}
\TODO{summarize this section}

\input{fig/star.tex}
\paragraph{Classical estimators}
%
We select two classical (pre-deep learning) methods to compare our solution against:
\CIRCLE{1} the VCM~\cite{merigot2011} method that uses the Voronoi covariance measure at a point for edge estimation;
\CIRCLE{2} EAR \citeN{huang2013} method, which performs edge-aware point cloud resampling.
\AT{in what way is (2) an edge estimator? this was not clear in the related works. AFAIR(emember) this method just resamples.}
% 
We consider these two methods representative of the state-of-the-art, as both have been adopted in the point-set processing routines of the popular CGAL library~\cite{cgal}.

For VCM method \cite{merigot2011}, we first compute Voronoi Covariance Measure for each point in the input point cloud. For parameters, we set offset radius 0.5 and convolution radius 0.25 which we found can lead algorithm to best performance in our testing dataset. We then compare Voronoi Covariance Measure of each point to a threshold. In this paper, We selected the best three thresholds ${0.12,0.17,0.22}$.

For EAR method \citeN{huang2013}, we first resample away from edges, leaving gaps near sharp edges using anisotroopic LOP. We set the parameters according to the EAR \citeN{huang2013}.
As the result, edge location are  emphasized by sparsity. 
So, we then calculate the average distance of the 10 nearest neighbors of each point in the point cloud. The longer the distance, the more likely it is to be an edge point.
we set the distance threshold from 0.1 to 0.5 with an interval 0.05, which determines whether a point is an edge point. 
Finally, we select three thresholds with best performance. 
The results are reported in Figure xxxx. our network can get more clear edge points, due to the fact that our network
can capture more richer edge feature information than non-learning methods.

\paragraph{Deep estimators}
We also compare our method against the recent EC-Net work in~\citeN{yu2018_ECNET} trained on our dataset. \AT{need to argue why we did not run our method on THEIR dataset?}

For EC-Net~\citeN{yu2018_ECNET}, since their dataset contained only 24 CAD models, the number is too small; and the edges were manually marked. It was difficult to use this dataset to train our network. So we used ABC dataset to generate training samples to train EC-NET. During the test phase, we use the same testing data as we did.

We report performanc on our dataset, as shown in Figure XXX. The results demonstrate the significant advantage of our network with better performance. 
Similarly, for edge points with less curvature, their method fails; At the same time, for small edge points, their network is difficult to get satisfactory results.

\paragraph{Comparison to SFPN}
\AT{?????} 

% \paragraph{Parameters}
% The core network parameters, if any, are: \rz{TBD}
% \AT{these are in the appendix}

==> 5_conclusions_OLD.tex <==
% \input{fig/limitation.tex}
% \paragraph{Limitations}
% Our current method still has some limitations, on which we see interesting directions for future works.
% \vspace{-.5em}
% \begin{itemize}[leftmargin=*]
%   \item First, our current network generates open curves based on corner pair sampling. For small curve segments, however, the two corner points can be very close to each other, it could be misjudged that there is no connectivity between the two corner pairs. Figure xxx (a) shows an example of such failure case. For such example, two small curve segments are missing. As a future work, we would liek to consider introducing an up-sampling module into our network to address this problem.
%   \item Figure xxx(b) shows another type of failure case. For closed curve generation, we first cluster the edge points, and then fit the closed curve according to the clustering results. When two closed curves are very close together, their clustering can be misleading, leading to only one closed curve being generated.
%   \item In addition, our method cannot deal with multi-mode problems, that is, there are multiple curves connecting two corners. In future work, it would be interesting to investigate how to extend our network to predict multiple curves for each corner pair.
% \end{itemize}

% %\AT{what happens if there are multiple paths within the sphere that connect the corners? Is this a limitation of the method? multi-modal inference is not trivial...}
% %\kx{This is a limitation and XG should put it in the limitation section.}



==> ablation.tex <==
\begin{table}[t]
\begin{overpic} 
[width=\linewidth]
{Images/radius_compare}
\end{overpic}
\vspace{-10pt}
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cc|cc|cc|c|c}
\hline
Metric   &  $R'= 1.5 \times R$   & $R'=3 \times R$    &  $\tau_c=0.8$  &  $\tau_c=0.95$  &  $\tau_c=0.6$  &  $\tau_c=0.8$  &  w/o $D_e$,$D_c$  & \textbf{\pie{} ($1 \times$, $0.9$, $0.7$) }\\
\hline\hline
ECD $\downarrow$  &   0.0326             &          0.0824        &             0.0150      &      0.0144    &           0.0163  &  0.0149  &  0.0186  &  \textbf{0.0136}    \\
IOU $\uparrow$  &  0.4386          &            0.2950           &            0.4875         &       0.5110  &     
0.4356  &  0.4964  &  0.5017  &  \textbf{0.5330} \\  
Precision $\uparrow$ & 0.5149         &             0.3244         &              0.5700     &       0.6032  &   
0.5180  &  0.5975  &  0.5824  &  \textbf{0.6219}  \\
Recall $\uparrow$ & 0.8570         &             \textbf{0.8910}         &              0.8415     &        0.8230   &
0.8340  &  0.8035  &  0.7849  &    0.8165       \\
\hline
\end{tabular}
} % resizebox
\end{center}
%\vspace{-1em}
\captionof{figure}{
% 
\textbf{Ablation studies} -- 
We evaluate the qualitative (top) and quantitative (bottom) performance of our method across a number of metrics as we tweak:
\CIRCLE{1} the sphere radius $R$ controlling our sampling heuristic~(\ali{\Section{proposal}})
\CIRCLE{2} the corner segmentation threshold $\tau_c$ (\Figure{patchnet}),
\CIRCLE{3} the edge segmentation threshold $\tau_e$ (\Figure{patchnet} and \Figure{closednet}) and
\CIRCLE{4} the edge and corner offsets $D_e$ and  $D_c$.
}
\label{fig:ablation}
\end{table}

==> fig/chair_and_table.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{Images/chair_and_table}
%\vspace{-2em}
\caption{\textbf{New Categories} --
xxxxxx.}
\label{fig:table_chair}
\end{figure*}

==> fig/chair_and_table_more.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{Images/chair_and_table_more}
%\vspace{-2em}
\caption{\textbf{Generalization to novel object categories} --
While \pie{} is trained on CAD models of mechanical assemblies from the ABC dataset~\cite{koch2019abc}, our edge detector is immediately applicable to 3D point clouds of general 3D objects and consistently outperforms VCM, EAR, and EC-Net.}
\label{fig:table_chair_more}
\end{figure*}

==> fig/closednet.tex <==
% \begin{figure*}[t]
% \centering
% \includegraphics[width=\textwidth]{Images/Closed_fit}
% %\vspace{-2em}
% \caption{\textbf{Closed curve proposal generation} -- We first identify the subset of points belonging to close curves via feature-based clustering and then fit a closed curve to each cluster. The network outputs both curve parameters and confidence scores.
% \AT{superimpose the point cloud to the output (with quasi-transparent color?}
% }
% \label{fig:closednet}
% \end{figure*}

==> fig/ecnet.tex <==
\begin{figure}
\centering
\begin{overpic} 
[width=\linewidth]
{fig/onecol.pdf}
\end{overpic}
%\vspace{-2em}
\caption{
\TODO{comparisons with ECNet}
}
\label{fig:deep}
\end{figure}

==> fig/limitation.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=3.4in]{Images/failure_case}
%\vspace{-2em}
\caption{\textbf{Limitations} --
% 
(left) Very short edges are at times missed by our method.
(right) Clustering might merge two curves into a single one.
We illustrate the \textit{missing} curves with dashed strokes.
%\AT{draw the missing curves with dashed lines? (instead of surrounding the mistakes with a dashed box)}
%\AT{super-impose the point cloud (transparent)?}
% 
}
\label{fig:limitations}
\end{figure}

==> fig/sampling.tex <==
\begin{figure}[!t]
\centering
\includegraphics[width=3.4in]{Images/corner_pair_sampling}
%\vspace{-2em}
\caption{\textbf{Corner pair sampling and segmentation} --
% 
Given a corner pair we only consider the samples between a sphere touching these points, and use a neural network to identify those points that describe a curve that start/ends at these corners.
% 
}
\label{fig:sampling}
\end{figure}

==> fig/sparse.tex <==
\begin{table}[t]
\begin{overpic} 
[width=\linewidth]
{Images/noise_dif}
\end{overpic}
\begin{center}
\resizebox{0.6\linewidth}{!}{
\begin{tabular}{l|c|c|c|c}
\hline
Metric   &  $P=1024$  &  $P=2048$  &  $P=4096$  &  $P=8096$\\
\hline\hline
ECD $\downarrow$   &  xxxxxx     &  xxxxxx     &  xxxxxx     &  0.0159   \\
IOU $\uparrow$     &  xxxxxx     &  xxxxxx     &  xxxxxx     &  0.6049   \\  
Precision $\uparrow$ &  xxxxxx   &  xxxxxx     &  xxxxxx     &  0.6672   \\
Recall $\uparrow$    &  xxxxxx   &  xxxxxx     &  xxxxxx     &  0.8691 \\
\hline
\end{tabular}
} % resizebox
\end{center}
%\vspace{-1em}
\captionof{figure}{
% 
\textbf{Noise data} -- 
We evaluate the qualitative (top) and quantitative (bottom) performance of the different number of point clouds: 
$P = \{1024, 2048, 4096, 8096\}$.
}
\label{fig:sparse}
\end{table}

==> fig/supp_all_methods.tex <==
\begin{figure*}[!t]
\centering
\includegraphics[width=\linewidth]{Images/all_edge_methods_1}
%\vspace{-2em}
\caption{\textbf{Comparisons to state-of-the-art methods} --
Qualitative comparisons against edge detection techniques -- VCM~\cite{merigot2011}, EAR~\cite{huang2013}, and EC-Net~\cite{yu2018_ECNET}.
}
\label{fig:supp_star}
\end{figure*}

==> fig/supp_para_curve.tex <==
\begin{figure*}[!t]
\centering
\includegraphics[width=\linewidth]{Images/more_results_1}
%\vspace{-2em}
\caption{Results on edge and corner detection and parametric curve inference by \pie{}.}
\label{fig:supp_para_curve}
\end{figure*}

==> future.tex <==
\section{Conclusion and future work}
\label{sec:future}


